Parameter-Free First-Order Method for Constrained Variational Inequalities

Constrained variational inequalities (VIs) provide a general framework for modeling and solving complementarity and equilibrium problems with functional constraints. In this paper, we propose a parameter-free accelerated operator sliding (PFAOS) method for solving monotone VIs with convex smooth constraints. For a single constraint, PFAOS achieves an operator evaluation complexity of $\mathcal{O}(1/\varepsilon)$ and a constraint gradient evaluation complexity of $\mathcal{O}(1/\sqrt{\varepsilon})$, without requiring prior knowledge of the Lipschitz constant of the VI operator or the smoothness constant of the constraint function. We further extend PFAOS to multiple constraints by incorporating a primal-dual hybrid gradient update, yielding a multi-constrained PFAOS (MC-PFAOS) method that preserves the same evaluation complexities. Finally, numerical experiments are conducted on large-scale games with coupling constraints to validate the efficiency and effectiveness of the proposed algorithms.

==> JoC_submission/results/mc_figures.tex <==
% MC-PFAOS versus projected OE: weak VI gap at n=100, m=1,000.
\begin{figure}[!htbp]
  \centering
  \includegraphics[width=0.7\linewidth]{JoC_submission/results/mc_ci_gap_comparison.pdf}
  \caption{Weak VI gap versus measured solver time for the
  $n=100$, $m=1000$ instance. The dashed line marks $10^{-5}$.}
  \label{fig:mc_gap_100_1000}
\end{figure}

% The same runs' coupling-constraint violation.
% \begin{figure}[!htbp]
%   \centering
%   \includegraphics[width=0.92\linewidth]{JoC_submission/results/mc_violation.pdf}
%   \caption{Positive constraint-violation norm for the same
%   multiple-constraint comparison.}
%   \label{fig:mc_violation_100_1000}
% \end{figure}


==> JoC_submission/results/mc_table.tex <==
% \begin{table*}[!htbp]
% \centering
% \caption{Time (seconds) to first independently certified $\operatorname{Gap}(\bar x_k)$ threshold at $n=1000$, and final constraint violation, over 10 normalized instances per constraint count. Entries give best, mean, and worst over seeds reaching the threshold; ``--'' means no seed produced a certified value within the 900-second cap. Each projection baseline rebuilds the complete generic projection at every iteration. Projected OE uses the true operator Lipschitz constant $M$, fixed throughout each run, and all four thresholds are extracted from that one trajectory.}
% \label{tab:multi_constraint_comparative}
% \setlength{\tabcolsep}{2.4pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clrrrrrrrrrrrrrrr}
% \hline
% $m$ & Method & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-2}$} & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-3}$} & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-4}$} & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-5}$} & \multicolumn{3}{c}{Final violation} \\
%  & & Best & Mean & Worst & Best & Mean & Worst & Best & Mean & Worst & Best & Mean & Worst & Best & Mean & Worst \\
% \hline
% \multirow{3}{*}{10} & MC-PFAOS & 0.87 & 1.34 & 1.61 & 3.72 & 6.28 & 8.55 & 13.70 & 49.87 & 241.68 & 87.49 & 689.89 & 885.96 & $3.11\times10^{-7}$ & $1.50\times10^{-6}$ & $8.98\times10^{-6}$ \\
%  & Projected OE (true M) & 41.72 & 74.31 & 88.45 & 407.70 & 714.90 & 850.09 & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
%  & Golden Ratio & 28.35 & 30.40 & 33.37 & 319.17 & 343.13 & 366.92 & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
% \hline
% \multirow{3}{*}{50} & MC-PFAOS & 0.27 & 1.20 & 1.60 & 2.41 & 5.72 & 8.07 & 44.13 & 217.36 & 625.65 & 106.62 & 493.29 & 639.35 & $7.76\times10^{-7}$ & $2.47\times10^{-6}$ & $7.16\times10^{-6}$ \\
%  & Projected OE (true M) & 129.67 & 146.02 & 223.67 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
%  & Golden Ratio & 88.12 & 93.26 & 98.77 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
% \hline
% \multirow{3}{*}{100} & MC-PFAOS & 0.76 & 1.37 & 1.88 & 5.17 & 8.54 & 14.51 & 39.71 & 95.68 & 140.15 & 270.20 & 602.77 & 814.72 & $9.46\times10^{-7}$ & $2.57\times10^{-6}$ & $3.82\times10^{-6}$ \\
%  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
%  & Golden Ratio & 346.97 & 396.00 & 457.09 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
% \hline
% \multirow{3}{*}{200} & MC-PFAOS & 0.64 & 1.50 & 2.92 & 4.43 & 13.54 & 22.32 & 80.16 & 192.78 & 336.82 & 497.75 & 640.20 & 776.31 & $1.18\times10^{-6}$ & $3.12\times10^{-6}$ & $8.58\times10^{-6}$ \\
%  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
%  & Golden Ratio & 604.88 & 672.00 & 745.22 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
% \hline
% \multirow{3}{*}{500} & MC-PFAOS & 4.99 & 7.46 & 9.50 & 18.58 & 34.48 & 51.81 & 143.18 & 380.74 & 731.63 & -- & -- & -- & $3.54\times10^{-6}$ & $1.04\times10^{-5}$ & $1.79\times10^{-5}$ \\
%  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
%  & Golden Ratio & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
% \hline
% \multirow{3}{*}{1000} & MC-PFAOS & 10.93 & 26.77 & 40.68 & 84.69 & 178.79 & 322.12 & 726.27 & 827.03 & 898.84 & -- & -- & -- & $6.87\times10^{-6}$ & $4.99\times10^{-5}$ & $8.23\times10^{-5}$ \\
%  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
%  & Golden Ratio & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
% \hline
% \end{tabular}%
% }
% \end{table*}


\begin{table*}[!htbp]
\centering
\caption{Time to first independently certified $\operatorname{Gap}(\bar x_k)$ threshold  and final constraint violation  over 10  instances.}
\label{tab:multi_constraint_comparative}
\setlength{\tabcolsep}{2.4pt}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{clrrrrrrrrrrrrrrr}
\hline
$m$ & Method & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-2}$} & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-3}$} & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-4}$} & \multicolumn{3}{c}{$\operatorname{Gap}\le10^{-5}$} & \multicolumn{3}{c}{Final violation} \\
  & & Best & Mean & Worst & Best & Mean & Worst & Best & Mean & Worst & Best & Mean & Worst & Best & Mean & Worst \\
\hline
\multirow{3}{*}{10} & MC-PFAOS & 0.87 & 1.34 & 1.61 & 3.72 & 6.28 & 8.55 & 13.70 & 49.87 & 241.68 & 87.49 & 689.89 & 885.96 & $3.11\times10^{-7}$ & $1.50\times10^{-6}$ & $8.98\times10^{-6}$ \\
  & Projected OE (true M) & 41.72 & 74.31 & 88.45 & 407.70 & 714.90 & 850.09 & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
  & Golden Ratio & 28.35 & 30.40 & 33.37 & 319.17 & 343.13 & 366.92 & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
\hline
\multirow{3}{*}{50} & MC-PFAOS & 0.27 & 1.20 & 1.60 & 2.41 & 5.72 & 8.07 & 44.13 & 217.36 & 625.65 & 106.62 & 493.29 & 639.35 & $7.76\times10^{-7}$ & $2.47\times10^{-6}$ & $7.16\times10^{-6}$ \\
  & Projected OE (true M) & 129.67 & 146.02 & 223.67 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
  & Golden Ratio & 88.12 & 93.26 & 98.77 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
\hline
\multirow{3}{*}{100} & MC-PFAOS & 0.76 & 1.37 & 1.88 & 5.17 & 8.54 & 14.51 & 39.71 & 95.68 & 140.15 & 270.20 & 602.77 & 814.72 & $9.46\times10^{-7}$ & $2.57\times10^{-6}$ & $3.82\times10^{-6}$ \\
  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
  & Golden Ratio & 346.97 & 396.00 & 457.09 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
\hline
\multirow{3}{*}{200} & MC-PFAOS & 0.64 & 1.50 & 2.92 & 4.43 & 13.54 & 22.32 & 80.16 & 192.78 & 336.82 & 497.75 & 640.20 & 776.31 & $1.18\times10^{-6}$ & $3.12\times10^{-6}$ & $8.58\times10^{-6}$ \\
  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
  & Golden Ratio & 604.88 & 672.00 & 745.22 & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
\hline
\multirow{3}{*}{500} & MC-PFAOS & 4.99 & 7.46 & 9.50 & 18.58 & 34.48 & 51.81 & 143.18 & 380.74 & 731.63 & -- & -- & -- & $3.54\times10^{-6}$ & $1.04\times10^{-5}$ & $1.79\times10^{-5}$ \\
  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
  & Golden Ratio & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
\hline
\multirow{3}{*}{1000} & MC-PFAOS & 10.93 & 26.77 & 40.68 & 84.69 & 178.79 & 322.12 & 726.27 & 827.03 & 898.84 & -- & -- & -- & $6.87\times10^{-6}$ & $4.99\times10^{-5}$ & $8.23\times10^{-5}$ \\
  & Projected OE (true M) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
  & Golden Ratio & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $0.00$ & $0.00$ & $0.00$ \\
\hline
\end{tabular}%
}
\smallskip
\parbox{\textwidth}{\footnotesize\textit{Note:} Fix $n=1000$, entries are normalized  per constraint count;
%and give best, mean, and worst over seeds reaching the threshold;
``--'' means no seed produced a certified value within the 900-second cap. 
%Each projection baseline rebuilds the complete generic projection at every iteration. 
Projected OE uses the true operator Lipschitz constant $M$.
%fixed throughout each run, and all four thresholds are extracted from that one trajectory.
}
\end{table*}

==> Literature.tex <==
\section{Literature Review} \label{sec:literature}

\subsection{First-Order Methods for Unconstrained VI}
Classical methods for monotone VIs combine operator evaluations
with projection or proximal updates.
\citet{korpelevich1976extragradient} introduced the extragradient
method and established its convergence for Lipschitz continuous
monotone operators.
Mirror-Prox \citep{nemirovski2004prox} and dual extrapolation
\citep{nesterov2007dual} achieve
$\mathcal O(1/\varepsilon)$ operator-evaluation complexity
for the weak VI gap of averaged iterates on bounded domains.
Forward-backward-forward splitting \citep{tseng2000modified}
uses one proximal evaluation and two operator evaluations
per iteration in its standard form.
Later methods require only one new operator evaluation per
iteration in their basic forms, including projected reflected
gradient \citep{malitsky2015projected},
forward-reflected-backward splitting \citep{malitsky2020forward},
and operator extrapolation \citep{kotsalis2020simplea}.
The adaptive golden ratio algorithm \citep{malitsky2020golden}
also adjusts step sizes without line searches.

For Lipschitz continuous monotone equations, fast optimistic
gradient descent-ascent (OGDA) \citep{bot2025fastogda} and
extragradient with flexible anchoring \citep{bot2026flexible}
achieve a last-iterate residual norm at most $\varepsilon$
using $\mathcal O(1/\varepsilon)$ operator evaluations
with suitable parameter choices.
\citet{upadhyaya2026lyapunov} sharpen extragradient's
last-iterate guarantees through a Lyapunov analysis.


\subsection{Computational Methods for  CVI}
\citet{boob2026firstorder} develop adaptive operator extrapolation
for smooth deterministic CVIs, achieving $\varepsilon$-accuracy
in both the weak VI gap and feasibility within
$\mathcal O(1/\varepsilon)$ iterations.
\citet{zhang2025primal} achieve these guarantees in
$\mathcal O(1/\varepsilon^2)$ iterations using local quadratic
programs, whose solution cost is additional to the operator-query bound.

Our methods build on gradient sliding for composite optimization
\citep{lan2016gradient} and acceleration for structured VIs
\citep{chen2017accelerated}.
For operators comprising a smooth convex gradient and a Lipschitz
monotone component, \citet{lan2021mirrorproxsliding} obtain an
$\varepsilon$-accurate weak solution using
$\mathcal O(1/\sqrt{\varepsilon})$ gradient evaluations and
$\mathcal O(1/\varepsilon)$ evaluations of the monotone component.

Related parameter-free developments include adaptive
past-extragradient methods \citep{ene2022adaptivevi}, which attain
$\mathcal O(1/\varepsilon)$ operator complexity for smooth
deterministic VIs on bounded domains.
\citet{deng2026uniformly} develop uniformly optimal methods
using quadratic-programming oracles, requiring
$\mathcal O(1/\sqrt{\varepsilon})$ function and gradient
evaluations for smooth function-constrained convex optimization.
\citet{wu2026universal} develop parameter-free gradient sliding
for composite optimization.
To our knowledge, our methods are the first to attain
$\mathcal O(1/\sqrt{\varepsilon})$ constraint-gradient evaluations
and $\mathcal O(1/\varepsilon)$ operator evaluations for smooth
monotone CVIs without prior knowledge of the Lipschitz
and smoothness constants.
